Handel: Practical Multi-Signature Aggregation for Large Byzantine Committees

We present Handel, a Byzantine-tolerant aggregation protocol that allows for the quick aggregation of cryptographic signatures over a WAN. Handel has polylogarithmic time, communication and processing complexity. We implemented Handel as an open source Go library with a flexible design to support any associative and commutative aggregation function. We tested Handel on 2000 AWS instances running two nodes per instance and located in 10 AWS regions. The 4000 signatures are aggregated in less than 900 milliseconds with an average per-node communication cost of 56KB.

==> diagrams/algo_disseminate.tex <==
\begin{algorithm}
\begin{algorithmic}[1]
\Procedure{Dissemination}{$.$}%\\\vspace{-12pt}
    \For{$level \gets 1 \dots level_{max}$}    
        \If{level started  or level completed}
            \State{c $\gets$ bestAggregatedContribution[level]}
            \State{send($level$,$c$,$1$)}
        \EndIf
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> diagrams/algo_scoring.tex <==
\begin{algorithm}
\begin{algorithmic}[1]
\Procedure{Score}{contribution, level}%\\\vspace{-12pt}
    \State{c $\gets$ contribution.cardinality}
    \If{c == 0}
        return 0
    \EndIf
    \If{level is complete}
        return 0
    \EndIf
    \State{augmented $\gets$ merge(contribution, individualContributions[level])}
    \If{augmented completes level}
        \State{return 1000 + level * 100}
    \EndIf
    \State{best $\gets$ bestAggregatedContribution[level]}
    \State{diff $\gets$ augmented.cardinality - best.cardinality}
    \If{(!canMerge(best, augmented)}
        \State{return level * 100 + diff * 10}
    \EndIf
    \State{merged $\gets$ merge(best,augmented)}
    \State{diff $\gets$ merged.cardinality - best.cardinality}
    \If{merged completes level}
        \State{return 1000 + level * 100}
    \EndIf
    \State{return level * 100 + diff * 10}
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> diagrams/algo_update.tex <==
\begin{algorithm}

\begin{algorithmic}[1]

\Procedure{UpdateLevels}{queue,nodeContribution,m}:
    \State{bestIncoming = queue.pickBest()}
    \State{ok $\gets$ verifyContribution(bestIncoming)}
    \If{not ok}
        \State{blacklist $\gets$ statement.identity}
        \State{\textbf{return}}
    \EndIf
     \State{bestIncoming.level.updateIncomingBestl(bestIncoming) }
    \For{$level \gets bestIncoming.level https://www.overleaf.com/project/5bc455a9f7f3ed6601785b6d+ 1 \dots level_{max}$}
        \State{level.updateOutcomingBest(bestIncoming) }
        \If{level is complete}
            \State{send(level,nodeContribution,m)}
        \EndIf
    \EndFor

\EndProcedure
\end{algorithmic}

\end{algorithm}

\iffalse
\section{First Verification Algo}
\begin{algorithm}
 \caption{Verification loop #1}

\begin{algorithmic}[1]

\Procedure{verificationLoop}{queue,m}:
    \State{maxScore $\gets$ 0}
    \State{maxStatement $\gets NULL$ }
      \For{queue not empty}
        \State{statement $\gets$ queue.pop()}
        \State{score $\gets$ score(statement)}
        \If{$score == 0$}
            \State{blacklist $\gets$ statement.identity}
        \ElsIf{$score > maxScore$}
            \State{maxScore $\gets$ score}
            \State{maxStatement $\gets$ statement}
        \EndIf
     \EndFor
    
    \For{$level \gets 1 \dots level_{max}$}
        \State{best $\gets$ bestStatement[level]}
        \State{best $\gets$ merge(best, maxStatement)}
        \State{bestStatement[level] $\gets$ best}
        \If{level.complete}
            \State{send(level,statement,m)}
        \EndIf
    \EndFor

\EndProcedure
\end{algorithmic}

\end{algorithm}
\\
\\
\section{Second Verification Algo}
\fi

==> diagrams/bin_forest.tex <==
\usetikzlibrary{shapes.symbols,decorations.text}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathreplacing}

\definecolor{nodecolor}{rgb}{0.03, 0.91, 0.87}
\definecolor{level1color}{rgb}{0.6, 0.98, 0.6}
\definecolor{level2color}{rgb}{0.31, 0.78, 0.47}
\definecolor{level3color}{rgb}{1.0, 0.87, 0.0}
\definecolor{level4color}{rgb}{1.0, 0.55, 0.41}

\def\vert{1}
\def\hori{1.2}
\def\outer{.53cm}
\def\inner{.75cm}
\def\factor{.90}

\begin{tikzpicture}
\def\n{4}
\foreach \i in {0,...,\n} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \pgfmathsetmacro\TwoToTheNMinusI{2^\n/2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \path
            (\TwoToTheNMinusI*\j*\hori-.5*\TwoToTheNMinusI*\hori,-\i*\vert)
                coordinate
                    (vertex=\i=\j);
    }
}
\pgfmathsetmacro\nRemoveOne{int(\n-1)}
\foreach \i in {0,...,\nRemoveOne} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \pgfmathsetmacro\nexti{int(\i+1)}
        \pgfmathsetmacro\l{int(2*\j-1)}
        \pgfmathsetmacro\r{int(2*\j)}
        \pgfmathsetmacro\Inti{int(\i)}
        \pgfmathsetmacro\Intj{int(\j)}
        \draw (vertex=\Inti=\Intj) -- (vertex=\nexti=\l);
        \draw (vertex=\Inti=\Intj) -- (vertex=\nexti=\r);
    }
}
\draw[draw=black, thick, fill=nodecolor!50] (vertex=4=6) circle(\outer);
%
\draw[draw=black, thick, fill=level1color] (vertex=4=5) circle(\outer);
%
\draw[draw=black, thick, fill=level2color] (vertex=4=7) circle(\outer);
\draw[draw=black, thick, fill=level2color] (vertex=4=8) circle(\outer);
%
\draw[draw=black, thick, fill=level3color] (vertex=4=1) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=4=2) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=4=3) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=4=4) circle(\outer);
%
\draw[draw=black, thick, fill=level4color] (vertex=4=9) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=10) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=11) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=12) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=13) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=14) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=15) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=16) circle(\outer);

\foreach \i in {0,...,\nRemoveOne} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \pgfmathsetmacro\TwoToTheNMinusI{2^\n/2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \pgfmathsetmacro\number{int(\TwoToTheI+\j-1)}
        \pgfmathsetmacro\Inti{int(\i)}
        \pgfmathsetmacro\Intj{int(\j)}
        \draw (vertex=\i=\j) node [circle, draw = black, fill = white] (vertex=\Inti=\Intj)  {\number};
    }
}
\pgfmathsetmacro\TwoToTheN{2^\n}
\foreach \j in {1,...,\TwoToTheN} {
    \pgfmathsetmacro\Intj{int(\j)}
    \pgfmathsetmacro\number{int(\j-1)}
    \draw (vertex=\n=\j) node [circle, draw = black, fill = white, inner sep=0pt, minimum size = \inner] {$\textsf{n}_{\number}$};
    %$\textsf{n}_{\number}$
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=6) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level -1 left) ;
\path   (vertex=4=6) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level -1 right) ;
\draw[decorate,decoration={brace,amplitude=7pt,mirror,raise=4pt},yshift=0pt]
    (level -1 left) -- (level -1 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_{-1}$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=5) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 0 left) ;
\path   (vertex=4=5) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 0 right) ;
\draw[decorate,decoration={brace,amplitude=7pt,mirror,raise=4pt},yshift=0pt]
    (level 0 left) -- (level 0 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_0$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=7) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 1 left) ;
\path   (vertex=4=8) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 1 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 1 left) -- (level 1 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_1$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=1) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 2 left) ;
\path   (vertex=4=4) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 2 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 2 left) -- (level 2 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_2$};           
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=9) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 3 left) ;
\path   (vertex=4=16) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 3 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 3 left) -- (level 3 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_3$};
\end{tikzpicture}

\begin{tikzpicture}
\def\n{4}
\foreach \i in {0,...,\n} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \pgfmathsetmacro\TwoToTheNMinusI{2^\n/2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \path
            (\TwoToTheNMinusI*\j*\hori-.5*\TwoToTheNMinusI*\hori,-\i*\vert)
                coordinate
                    (vertex=\i=\j);
    }
}
\pgfmathsetmacro\nRemoveOne{int(\n-1)}
\foreach \i in {0,...,\nRemoveOne} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \pgfmathsetmacro\nexti{int(\i+1)}
        \pgfmathsetmacro\l{int(2*\j-1)}
        \pgfmathsetmacro\r{int(2*\j)}
        \pgfmathsetmacro\Inti{int(\i)}
        \pgfmathsetmacro\Intj{int(\j)}
        \draw (vertex=\Inti=\Intj) -- (vertex=\nexti=\l);
        \draw (vertex=\Inti=\Intj) -- (vertex=\nexti=\r);
    }
}
\draw[draw=black, thick, fill=nodecolor!50] (vertex=4=6) circle(\outer);
%
\draw[draw=black, thick, fill=level1color] (vertex=4=5) circle(\outer);
%
\draw[draw=black, thick, fill=level2color] (vertex=4=7) circle(\outer);
\draw[draw=black, thick, fill=level2color] (vertex=4=8) circle(\outer);
%
\draw[draw=black, thick, fill=level3color] (vertex=4=1) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=4=2) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=4=3) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=4=4) circle(\outer);
%
\draw[draw=black, thick, fill=level4color] (vertex=4=9) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=10) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=11) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=12) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=13) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=14) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=15) circle(\outer);
\draw[draw=black, thick, fill=level4color] (vertex=4=16) circle(\outer);

\foreach \i in {0,...,\nRemoveOne} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \pgfmathsetmacro\TwoToTheNMinusI{2^\n/2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \pgfmathsetmacro\number{int(\TwoToTheI+\j-1)}
        \pgfmathsetmacro\Inti{int(\i)}
        \pgfmathsetmacro\Intj{int(\j)}
        \draw (vertex=\i=\j) node [circle, draw = black, fill = white] (vertex=\Inti=\Intj)  {\number};
    }
}
\pgfmathsetmacro\TwoToTheN{2^\n}
\foreach \j in {1,...,\TwoToTheN} {
    \pgfmathsetmacro\Intj{int(\j)}
    \pgfmathsetmacro\number{int(\j-1)}
    \draw (vertex=\n=\j) node [circle, draw = black, fill = white, inner sep=0pt, minimum size = \inner] {$\textsf{n}_{\number}$};
    %$\textsf{n}_{\number}$
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=6) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level -1 left) ;
\path   (vertex=4=6) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level -1 right) ;
\draw[decorate,decoration={brace,amplitude=7pt,mirror,raise=4pt},yshift=0pt]
    (level -1 left) -- (level -1 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_{-1}$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=5) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 0 left) ;
\path   (vertex=4=5) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 0 right) ;
\draw[decorate,decoration={brace,amplitude=7pt,mirror,raise=4pt},yshift=0pt]
    (level 0 left) -- (level 0 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_0$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=7) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 1 left) ;
\path   (vertex=4=8) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 1 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 1 left) -- (level 1 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_1$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=1) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 2 left) ;
\path   (vertex=4=4) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 2 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 2 left) -- (level 2 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_2$};           
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=4=9) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 3 left) ;
\path   (vertex=4=16) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 3 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 3 left) -- (level 3 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_3$};
\end{tikzpicture}


\begin{tikzpicture}
\def\n{3}
\foreach \i in {0,...,\n} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \pgfmathsetmacro\TwoToTheNMinusI{2^\n/2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \path
            (\TwoToTheNMinusI*\j*\hori-.5*\TwoToTheNMinusI*\hori,-\i*\vert)
                coordinate
                    (vertex=\i=\j);
    }
}
\pgfmathsetmacro\nRemoveOne{int(\n-1)}
\foreach \i in {0,...,\nRemoveOne} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \pgfmathsetmacro\nexti{int(\i+1)}
        \pgfmathsetmacro\l{int(2*\j-1)}
        \pgfmathsetmacro\r{int(2*\j)}
        \pgfmathsetmacro\Inti{int(\i)}
        \pgfmathsetmacro\Intj{int(\j)}
        \draw (vertex=\Inti=\Intj) -- (vertex=\nexti=\l);
        \draw (vertex=\Inti=\Intj) -- (vertex=\nexti=\r);
    }
}
\draw[draw=black, thick, fill=nodecolor!50] (vertex=\n=6) circle(\outer);
%
\draw[draw=black, thick, fill=level1color] (vertex=\n=5) circle(\outer);
%
\draw[draw=black, thick, fill=level2color] (vertex=\n=7) circle(\outer);
\draw[draw=black, thick, fill=level2color] (vertex=\n=8) circle(\outer);
%
\draw[draw=black, thick, fill=level3color] (vertex=\n=1) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=\n=2) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=\n=3) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=\n=4) circle(\outer);

\foreach \i in {0,...,\nRemoveOne} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \pgfmathsetmacro\TwoToTheNMinusI{2^\n/2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \pgfmathsetmacro\number{int(\TwoToTheI+\j-1)}
        \pgfmathsetmacro\Inti{int(\i)}
        \pgfmathsetmacro\Intj{int(\j)}
        \draw (vertex=\i=\j) node [circle, draw = black, fill = white] (vertex=\Inti=\Intj)  {\number};
    }
}
\pgfmathsetmacro\TwoToTheN{2^\n}
\foreach \j in {1,...,\TwoToTheN} {
    \pgfmathsetmacro\Intj{int(\j)}
    \pgfmathsetmacro\number{int(\j-1)}
    \draw (vertex=\n=\j) node [circle, draw = black, fill = white, inner sep=0pt, minimum size = \inner] {$\textsf{n}_{\number}$};
    %$\textsf{n}_{\number}$
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=\n=6) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level -1 left) ;
\path   (vertex=\n=6) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level -1 right) ;
\draw[decorate,decoration={brace,amplitude=7pt,mirror,raise=4pt},yshift=0pt]
    (level -1 left) -- (level -1 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_{-1}$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=\n=5) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 0 left) ;
\path   (vertex=\n=5) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 0 right) ;
\draw[decorate,decoration={brace,amplitude=7pt,mirror,raise=4pt},yshift=0pt]
    (level 0 left) -- (level 0 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_0$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=\n=7) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 1 left) ;
\path   (vertex=\n=8) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 1 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 1 left) -- (level 1 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_1$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=\n=1) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 2 left) ;
\path   (vertex=\n=4) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 2 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 2 left) -- (level 2 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_2$};
\end{tikzpicture}


\begin{tikzpicture}
\def\n{3}
\foreach \i in {0,...,\n} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \pgfmathsetmacro\TwoToTheNMinusI{2^\n/2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \path
            (\TwoToTheNMinusI*\j*\hori-.5*\TwoToTheNMinusI*\hori,-\i*\vert)
                coordinate
                    (vertex=\i=\j);
    }
}
\pgfmathsetmacro\nRemoveOne{int(\n-1)}
\foreach \i in {0,...,\nRemoveOne} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \pgfmathsetmacro\nexti{int(\i+1)}
        \pgfmathsetmacro\l{int(2*\j-1)}
        \pgfmathsetmacro\r{int(2*\j)}
        \pgfmathsetmacro\Inti{int(\i)}
        \pgfmathsetmacro\Intj{int(\j)}
        \draw (vertex=\Inti=\Intj) -- (vertex=\nexti=\l);
        \draw (vertex=\Inti=\Intj) -- (vertex=\nexti=\r);
    }
}
\draw[draw=black, thick, fill=nodecolor!50] (vertex=\n=6) circle(\outer);
%
\draw[draw=black, thick, fill=level1color] (vertex=\n=5) circle(\outer);
%
\draw[draw=black, thick, fill=level2color] (vertex=\n=7) circle(\outer);
\draw[draw=black, thick, fill=level2color] (vertex=\n=8) circle(\outer);
%
\draw[draw=black, thick, fill=level3color] (vertex=\n=1) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=\n=2) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=\n=3) circle(\outer);
\draw[draw=black, thick, fill=level3color] (vertex=\n=4) circle(\outer);

\foreach \i in {0,...,\nRemoveOne} {
    \pgfmathsetmacro\TwoToTheI{2^\i}
    \pgfmathsetmacro\TwoToTheNMinusI{2^\n/2^\i}
    \foreach \j in {1,...,\TwoToTheI} {
        \pgfmathsetmacro\number{int(\TwoToTheI+\j-1)}
        \pgfmathsetmacro\Inti{int(\i)}
        \pgfmathsetmacro\Intj{int(\j)}
        \draw (vertex=\i=\j) node [circle, draw = black, fill = white] (vertex=\Inti=\Intj)  {\number};
    }
}
\pgfmathsetmacro\TwoToTheN{2^\n}
\foreach \j in {1,...,\TwoToTheN} {
    \pgfmathsetmacro\Intj{int(\j)}
    \pgfmathsetmacro\number{int(\j-1)}
    \draw (vertex=\n=\j) node [circle, draw = black, fill = white, inner sep=0pt, minimum size = \inner] {$\textsf{n}_{\number}$};
    %$\textsf{n}_{\number}$
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=\n=6) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level -1 left) ;
\path   (vertex=\n=6) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level -1 right) ;
\draw[decorate,decoration={brace,amplitude=7pt,mirror,raise=4pt},yshift=0pt]
    (level -1 left) -- (level -1 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_{-1}$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=\n=5) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 0 left) ;
\path   (vertex=\n=5) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 0 right) ;
\draw[decorate,decoration={brace,amplitude=7pt,mirror,raise=4pt},yshift=0pt]
    (level 0 left) -- (level 0 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_0$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=\n=7) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 1 left) ;
\path   (vertex=\n=8) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 1 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 1 left) -- (level 1 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_1$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\path   (vertex=\n=1) ++ (-\factor*\outer, -\factor*\outer)
            coordinate (level 2 left) ;
\path   (vertex=\n=4) ++ (\factor*\outer, -\factor*\outer)
            coordinate (level 2 right) ;
\draw[decorate,decoration={brace,amplitude=10pt,mirror,raise=4pt},yshift=0pt]
    (level 2 left) -- (level 2 right)
        node[black,midway, yshift = -.75cm]
            {$\displaystyle C^{\textsf{n}_5}_2$};
\end{tikzpicture}

==> diagrams/forest.tex <==

\begin{tikzpicture}
%\newcount\myX
%\newcount\offsetY % each level moves by this offset
%\offsetY = 2
%\newcount\offsetX % each circles starts at this given x offset
%\offsetX = 2
\newcount\ycoord;
%\newcount\lastX % storing the y-coordinate of the whole level graphics
%\newcount\groupBy % how many circle the ellipsis should group by
%\COPY{0.9}{\ellipseRad}; % store radius inside the \radius variable
%\COPY{0.5}{\circleRad};
% level 0
\ycoord = \numexpr(\offsetY * 0)\relax;
\draw [font=\bfseries] (0,\ycoord) -- (0,\ycoord) node {\large Level 0};

\colorlet{ellipsColor}{gray!30!white}
\colorlet{circleColor}{orange!40!white}

%% increment of 2.5 for each node xcoord
\filldraw[fill=ellipsColor, thick] (2,\ycoord) circle [x radius=0.9, y radius=0.7];
\filldraw[fill=circleColor,thick,draw=black] (2,\ycoord) circle [radius=0.5] node {\large 00};

\filldraw[fill=ellipsColor, thick] (4.5,\ycoord) circle [x radius=0.9, y radius=0.7];
\filldraw[fill=circleColor, thick,draw=black] (4.5,\ycoord) circle [radius=0.5] node {\large 01};

\filldraw[fill=ellipsColor, thick] (7,\ycoord) circle [x radius=0.9, y radius=0.7];
\filldraw[fill=circleColor,thick,draw=black] (7,\ycoord) circle [radius=0.5] node {\large 10};

\filldraw[fill=ellipsColor, thick] (9.5,\ycoord) circle [x radius=0.9, y radius=0.7];
\filldraw[fill=circleColor,thick,draw=black] (9.5,\ycoord) circle [radius=0.5] node {\large 11};

%\foreach \id [count=\x from 0] in {{00},{01},{10},{11}} {
%    \myX = \numexpr(\offsetX + \x * 3)\relax;
%   \filldraw[fill=gray!20!white, thick] (\myX,\ycoord) circle [x radius=\ellipseRad, y radius=0.7];
%    \draw[thick,black] (\myX,\ycoord) circle [radius=\circleRad] node {\id};
%}


% level 1

%\lastX = 0
%\groupBy = 2
%\ycoord = \numexpr(\offsetY * 1)\relax;
\ycoord = 2
\COPY{1.7}{\y1}
\draw [font=\bfseries] (0,\y1) -- (0,\y1) node {\large Level 1};

% (2 + 4.5) / 2 = 3.25
\filldraw[fill=ellipsColor, thick] (3.25,\y1) circle [x radius=2.0, y radius=0.9];
\filldraw [fill=circleColor,thick,draw=black] (2,\y1) circle [radius=0.5] node {\large 00};
\filldraw [fill=circleColor,thick,draw=black,] (4.5,\y1) circle [radius=0.5] node {\large 01};

\filldraw[fill=ellipsColor, thick] (8.25,\y1) circle [x radius=2.0, y radius=0.9];
\filldraw[fill=circleColor,thick,draw=black] (7,\y1) circle [radius=0.5] node {\large 10};
\filldraw[fill=circleColor,thick,draw=black] (9.5,\y1) circle [radius=0.5] node {\large 11};


\COPY{3.9}{\y2}
\draw [font=\bfseries] (0,\y2) -- (0,\y2) node {\large Level 2};

\filldraw[fill=ellipsColor, thick] (5.75,\y2) circle [x radius=4.7, y radius=1.1];
\filldraw [fill=circleColor,thick,draw=black] (2,\y2) circle [radius=0.5] node {\large 00};
\filldraw [fill=circleColor,thick,draw=black] (4.5,\y2) circle [radius=0.5] node {\large 01};
\filldraw[fill=circleColor,thick,draw=black] (7,\y2) circle [radius=0.5] node { \large 10};
\filldraw[fill=circleColor,thick,draw=black] (9.5,\y2) circle [radius=0.5] node {\large 11};

% legend

\COPY{5.8}{\legendY}
\COPY{3.0}{\legendX}
\filldraw[fill=circleColor,thick,draw=black] (\legendX,\legendY) circle [radius=0.5] node[anchor=east,outer sep=15] {\large Node ID};
\ADD{\legendX}{5.8}{\legendX}
\filldraw[fill=ellipsColor, thick] (\legendX,\legendY) circle [x radius=0.5, y radius=0.5] node[anchor=east,outer sep=15, align=left] {\large Aggregated Contribution};

%\foreach \id [count=\x from 0] in {{00},{01},{10},{11}} {
%    \myX = \numexpr(\offsetX + \x * 2)\relax;
    %\ifnum \lastX=0\relax
        %\laxtX=\myX;
    %\fi
    %\MODULO{\numexpr(\x + 1)}{\groupBy}{\boundary}; % (x+1) mod groupBy
    %\ifnum\boundary=0 
    %    % compute x coordinates of the ellipsis
    %    
    %    \filldraw[fill=gray!20!white, thick] (\lastX,\ycoord) circle [x radius=0.9, y radius=0.7];
    %\fi
%    \filldraw[fill=gray!20!white, thick] (\lastX,\ycoord) circle [x radius=0.9, y radius=0.7];
%    \draw [thick,black] (\myX,\ycoord) circle [radius=0.5] node {\id};
%}


%\foreach \id [count=\x from 0] in {{00},{01},{10},{11}}
%    \myX = \numexpr(\x * 2)\relax;
%    \draw[thick] (\myX,0) circle [x radius=0.9, y radius=0.7];
%    \draw[thick, black] (\myX,6) circle [radius=0.5]  node {\id};
    


%\draw[thick,black] (0,0) circle [radius=2];

%\draw (0,0) rectangle (4,4);

%\draw (0,0) parabola (4,4);

%\draw (0,0) .. controls (0,4) and (4,0) .. (4,4);

%\draw[red,thick,dashed] (2,2) circle (3cm);

%\draw (2,2) ellipse (3cm and 1cm);

%\draw (3,0) arc (0:75:3cm);

%\draw[step=1cm,gray,very thin] (-1.9,-1.9) grid (5.9,5.9);

%\shadedraw[inner color=blue,outer color=red, draw=black] (0,0) rectangle (4,4);

%\draw[thick,->] (0,0) -- (4.5,0) node[anchor=north west] {x axis};
%\draw[thick,->] (0,0) -- (0,4.5) node[anchor=south east] {y axis};

%\foreach \x in {0,1,2,3,4}
%    \draw (\x cm,1pt) -- (\x cm,-1pt) node[anchor=north] {$\x$};
%\foreach \y in {0,1,2,3,4}
%    \draw (1pt,\y cm) -- (-1pt,\y cm) node[anchor=east] {$\y$};

\end{tikzpicture}

==> diagrams/types_level.tex <==
\noindent\textbf{Level}\{\\\vspace{0pt}
\begin{tabular}{ll}
\quad\textbf{id}~:&      Integer\\
\quad\textbf{best}~:&    Contribution\\
\quad\textbf{peers}~:&   CircularArray[Node]\\
\quad\textbf{sendPos}~:& Integer\\
\end{tabular}\\\vspace{0pt}
\noindent\}\\\vspace{20pt}

==> diagrams/types_message.tex <==
\noindent\textbf{Message}\{\\\vspace{0pt}
\begin{tabular}{ll}
\quad\textbf{levelNumber}~:&           Integer\\
\quad\textbf{individualContribution}~:& Contribution\\
\quad\textbf{contributionIncluded}~:& BitSet\\
\quad\textbf{aggregatedContribution}~:& Contribution\\
\end{tabular}\\\vspace{0pt}
\noindent\}\\\vspace{20pt}
